Nerfies: Deformable Neural Radiance Fields

We present the first method capable of photorealistically reconstructing deformable scenes using photos/videos captured casually from mobile phones. Our approach augments neural radiance fields (NeRF) by optimizing an additional continuous volumetric deformation field that warps each observed point into a canonical 5D NeRF. We observe that these NeRF-like deformation fields are prone to local minima, and propose a coarse-to-fine optimization method for coordinate-based models that allows for more robust optimization. By adapting principles from geometry processing and physical simulation to NeRF-like models, we propose an elastic regularization of the deformation field that further improves robustness. We show that our method can turn casually captured selfie photos/videos into deformable NeRF models that allow for photorealistic renderings of the subject from arbitrary viewpoints, which we dub "nerfies." We evaluate our method by collecting time-synchronized data using a rig with two mobile phones, yielding train/validation images of the same pose at different viewpoints. We show that our method faithfully reconstructs non-rigidly deforming scenes and reproduces unseen views with high fidelity.

==> f0x_latent_interpolation.tex <==
% \setlength{\fboxrule}{2pt}
% \setlength{\fboxsep}{0pt}
% \begin{figure}[t]
% 	\centering
% 	\begin{tabular}{@{}c@{\,\,\,}c@{\,\,\,}c@{}}
%     \fbox{\includegraphics[height=9.8mm]{figures/latent_interpolation/left_right_start.png}}&
%     \includegraphics[height=9.8mm]{figures/latent_interpolation/left_right_v2.png}&
%     \fbox{\includegraphics[height=9.8mm]{figures/latent_interpolation/left_right_end.png}}
%     \end{tabular}
%     \vspace{-8pt}
% 	\caption{
% 	Novel views synthesized (middle) by linearly interpolating the observation latent codes between two captures (left and right). The generated views recreate a smooth deformation field akin to a natural head pose rotation.
% 	}
%     \vspace{-5pt}
%   \label{fig:latent_interpolation}
% \end{figure}


\fboxsep=0pt % padding thickness
\fboxrule=1pt % border thickness

\definecolor{startcolor}{rgb}{0.067, 0.541, 0.698}
\definecolor{endcolor}{rgb}{0.937, 0.278, 0.435}
% \definecolor{startcolor}{rgb}{0.953, 0.447, 0.173}
% \definecolor{endcolor}{rgb}{0.937, 0.278, 0.435}

\newcommand{\kfbox}[1]{\fcolorbox{black}{white}{#1}}
\newcommand{\kfboxstart}[1]{\fcolorbox{startcolor}{white}{#1}}
\newcommand{\kfboxend}[1]{\fcolorbox{endcolor}{white}{#1}}
\newcommand{\latcell}[1]{\includegraphics[width=1.2cm,clip,trim=60 170 40 100]{#1}}
\newcommand{\latcellkfstart}[1]{\kfboxstart{\includegraphics[width=1.2cm,clip,trim=60 170 40 100]{#1}}}
\newcommand{\latcellkfend}[1]{\kfboxend{\includegraphics[width=1.2cm,clip,trim=60 170 40 100]{#1}}}

\begin{figure}[t]
    \setlength{\tabcolsep}{0.5pt}
    \renewcommand{\arraystretch}{0.25}
    \centering
    \begin{tabular}{ccccccc}
    
        \multirow{4}*[1.0cm]{\kfboxstart{\includegraphics[width=0.93cm,clip,trim=60 0 40 0]{figures/interp/00_000582.png}}\hspace{0.05cm}} &
        
        % \makebox[12pt]{\raisebox{23pt}{\rotatebox[origin=c]{90}{no elastic}}} \hspace{-3pt} &
        \latcellkfstart{figures/interp/noarap/interp_00.png} &
        \latcell{figures/interp/noarap/interp_01.png} &
        \latcell{figures/interp/noarap/interp_02.png} &
        \latcell{figures/interp/noarap/interp_03.png} &
        \latcellkfend{figures/interp/noarap/interp_04.png} &
        
        \multirow{4}*[1.0cm]{\hspace{0.05cm}\kfboxend{\includegraphics[width=0.93cm,clip,trim=60 0 40 0]{figures/interp/01_000651.png}}}
        \vspace{2pt}
        \\
        
        & 
        \multicolumn{5}{c}{{\footnotesize interpolation w/o elastic regularization}} &         \vspace{1pt}

        \\
       
       
        {\footnotesize start}
            % \makebox[12pt]{\raisebox{23pt}{\rotatebox[origin=c]{90}{elastic}}} \hspace{-3pt} &
        &
        \latcellkfstart{figures/interp/arap/interp_00.png} &
        \latcell{figures/interp/arap/interp_01.png} &
        \latcell{figures/interp/arap/interp_02.png} &
        \latcell{figures/interp/arap/interp_03.png} &
        \latcellkfend{figures/interp/arap/interp_04.png} & 
        
        {\footnotesize end}
        \vspace{2pt}
        \\
        & \multicolumn{5}{c}{{\footnotesize interpolation w/ elastic regularization}} & 
        %\\
        % \makebox[12pt]{\raisebox{23pt}{\rotatebox[origin=c]{90}{target}}} \hspace{-5pt} 
        
        % &
    \end{tabular}
    \vspace{-10pt}
	\caption{
	    Novel views synthesized without and with elastic regularization by linearly interpolating observation deformation codes (keyframes are \kfbox{outlined}). Without elastic regularization, intermediate states show distortions.
	}
  \label{fig:latent_interpolation}
  \vspace{-8pt}
\end{figure}


==> fa0_vrig_results_combined.tex <==
\definecolor{bestcolor}{rgb}{0.85, 0.113, 0.188}


\renewcommand{\textimage}[4]{
	\begin{overpic}[width=2.35cm,unit=1mm,clip,trim=#1]{figures/vrig_results_v3/#2}
	\put (9.9,0.7) {\sethlcolor{white}\footnotesize\hl{$#3 / #4$}}
    \end{overpic}
}
\newcommand{\textimagelonger}[4]{
	\begin{overpic}[width=2.35cm,unit=1mm,clip,trim=#1]{figures/vrig_results_v3/#2}
	\put (8.5,0.7) {\sethlcolor{white}\footnotesize\hl{$#3 / #4$}}
    \end{overpic}
}

\newcommand{\animage}[2]{\includegraphics[width=2.35cm,clip,trim=#1]{figures/vrig_results_v2/#2}}
\newcommand{\bestnum}[1]{\textcolor{bestcolor}{#1}}


\begin{figure*}[t!]
    \setlength{\tabcolsep}{0.5pt}
    \renewcommand{\arraystretch}{0.25}
    \begin{tabular}{cccccccc}
        % \makebox[20pt]{\raisebox{50pt}{\rotatebox[origin=c]{90}{\textsc{Drinking}}}} \hspace{-7pt} &
        % \animage{0 0 0 0}{drinking-from-cup1.train.jpg} &
        % \animage{0 0 0 0}{drinking-from-cup1.valid.jpg} &
        % \textimagelonger{0 0 0 0}{drinking-from-cup1.full_model_se3_w0.01.pred.jpg}{22.6}{\bestnum{0.0826}} &
        % \textimage{0 0 0 0}{drinking-from-cup1.d-nerf.pred.jpg}{\bestnum{25.7}}{0.156} &
        % \textimage{0 0 0 0}{drinking-from-cup1.nsff.pred.jpg}{{24.2}}{0.158} &
        % \textimage{0 0 0 0}{drinking-from-cup1.neuralvolumes.pred.jpg}{16.6}{0.183} &
        % \textimage{0 0 0 0}{drinking-from-cup1.nerf.pred.jpg}{20.1}{0.379} \\
        
        %     \makebox[20pt]{\raisebox{50pt}{\rotatebox[origin=c]{90}{\textsc{Glasses}}}} \hspace{-7pt} &
        % \animage{0 0 0 0}{keunhong-vrig4.train.jpg} &
        % \animage{0 0 0 0}{keunhong-vrig4.valid.jpg} &
        % \textimage{0 0 0 0}{keunhong-vrig4.full_model_se3_w0.01.pred.jpg}{\bestnum{22.1}}{\bestnum{0.329}} &
        % \textimage{0 0 0 0}{keunhong-vrig4.d-nerf.pred.jpg}{19.3}{0.417} &
        % \textimage{0 0 0 0}{keunhong-vrig4.nsff.pred.jpg}{14.0}{0.570} &
        % \textimage{0 0 0 0}{keunhong-vrig4.neuralvolumes.pred.jpg}{14.2}{0.660} &
        % \textimage{0 0 0 0}{keunhong-vrig4.nerf.pred.jpg}{15.5}{0.543} \\
        
        % \makebox[20pt]{\raisebox{45pt}{\rotatebox[origin=c]{90}{\textsc{Beanie}}}} \hspace{-7pt} &
        % \animage{0 0 0 0}{haley-vrig-beanie.train.jpg} &
        % \animage{0 0 0 0}{haley-vrig-beanie.valid.jpg} &
        % \textimage{0 0 0 0}{haley-vrig-beanie.full_model_se3.pred.jpg}{\bestnum{21.4}}{\bestnum{0.416}} &
        % \textimage{0 0 0 0}{haley-vrig-beanie.d-nerf.pred.jpg}{17.1}{0.512} &
        % \textimage{0 0 0 0}{haley-vrig-beanie.nsff.pred.jpg}{17.6}{0.513} &
        % \textimage{0 0 0 0}{haley-vrig-beanie.neuralvolumes.pred.jpg}{16.3}{0.573} &
        % \textimage{0 0 0 0}{haley-vrig-beanie.nerf.pred.jpg}{13.5}{0.667} \\
        
        \makebox[20pt]{\raisebox{50pt}{\rotatebox[origin=c]{90}{\textsc{Curls}}}} \hspace{-7pt} &
        \animage{0 0 0 40}{keunhong-vrig-bookshelf.train.jpg} &
        \animage{0 0 0 40}{keunhong-vrig-bookshelf.valid.jpg} &
        \textimage{0 0 0 80}{keunhong-vrig-bookshelf.full_model_se3.pred.jpg}{\bestnum{26.2}}{\bestnum{0.250}} &
        \textimage{0 0 0 80}{keunhong-vrig-bookshelf.d-nerf.pred.jpg}{23.3}{0.357} &
        \textimage{0 0 0 80}{keunhong-vrig-bookshelf.nsff.pred.jpg}{15.6}{0.552} &
        \textimage{0 0 0 80}{keunhong-vrig-bookshelf.neuralvolumes.pred.jpg}{15.1}{0.576} &
        \textimage{0 0 0 80}{keunhong-vrig-bookshelf.nerf.pred.jpg}{12.8}{0.657} \\
        
        % \makebox[20pt]{\raisebox{45pt}{\rotatebox[origin=c]{90}{\textsc{Kitchen}}}} \hspace{-7pt} &
        % \animage{0 0 0 0}{aleks-vrig3-v2.train.jpg} &
        % \animage{0 0 0 0}{aleks-vrig3-v2.valid.jpg} &
        % \textimage{0 0 0 0}{aleks-vrig3-v2.full_model_se3_w0.01.pred.jpg}{\bestnum{25.6} }{\bestnum{0.277}} &
        % \textimage{0 0 0 0}{aleks-vrig3-v2.d-nerf.pred.jpg}{22.4}{0.350} &
        % \textimage{0 0 0 0}{aleks-vrig3-v2.nsff.pred.jpg}{22.0}{0.428} &
        % \textimage{0 0 0 0}{aleks-vrig3-v2.neuralvolumes.pred.jpg}{17.2}{0.571} &
        % \textimage{0 0 0 0}{aleks-vrig3-v2.nerf.pred.jpg}{20.8}{0.393} \\
         
        % \makebox[20pt]{\raisebox{50pt}{\rotatebox[origin=c]{90}{\textsc{Lamp}}}} \hspace{-7pt} &
        % \animage{0 0 0 0}{yash-vrig-mask.train.jpg} &
        % \animage{0 0 0 0}{yash-vrig-mask.valid.jpg} &
        % \textimage{0 0 0 0}{yash-vrig-mask.full_model_se3.pred.jpg}{\bestnum{20.7}}{\bestnum{0.258}} &
        % \textimage{0 0 0 0}{yash-vrig-mask.d-nerf.pred.jpg}{18.0}{0.336} &
        % \textimage{0 0 0 0}{yash-vrig-mask.nsff.pred.jpg}{18.3}{0.347} &
        % \textimage{0 0 0 0}{yash-vrig-mask.neuralvolumes.pred.jpg}{14.2}{0.523} &
        % \textimage{0 0 0 0}{yash-vrig-mask.nerf.pred.jpg}{17.5}{0.438} \\
        
        \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{90}{\textsc{Toby Sit}}}} \hspace{-7pt} &
        \animage{70 140 20 20}{toby-sit-outside1.train.jpg} &
        \animage{50 140 40 20}{toby-sit-outside1.valid.jpg} &
        \textimage{50 140 40 20}{toby-sit-outside1.full_model_se3.pred.jpg}{23.2}{\bestnum{0.143}} &
        \textimage{50 140 40 20}{toby-sit-outside1.d-nerf.pred.jpg}{\bestnum{25.6}}{0.435} &
        \textimage{50 140 40 20}{toby-sit-outside1.nsff.pred.jpg}{25.5}{0.285} &
        \textimage{50 140 40 20}{toby-sit-outside1.neuralvolumes.pred.jpg}{{13.4}}{0.488} &
        \textimage{50 140 40 20}{toby-sit-outside1.nerf.pred.jpg}{22.2}{0.469} \\
        
        \makebox[20pt]{\raisebox{45pt}{\rotatebox[origin=c]{90}{\textsc{badminton}}}} \hspace{-7pt} &
        \animage{30 90 30 50}{badminton1.train.jpg} &
        \animage{30 90 30 50}{badminton1.valid.jpg} &
        \textimage{30 90 30 50}{badminton1.full_model_se3_w0.01.pred.jpg}{22.4}{\bestnum{0.118}} &
        \textimage{30 90 30 50}{badminton1.d-nerf.pred.jpg}{\bestnum{22.9}}{0.198} &
        \textimage{30 90 30 50}{badminton1.nsff.pred.jpg}{17.0}{0.390} &
        \textimage{30 90 30 50}{badminton1.neuralvolumes.pred.jpg}{{13.1}}{0.520} &
        \textimage{30 90 30 50}{badminton1.nerf.pred.jpg}{19.5}{0.360} \\
        
        % \makebox[20pt]{\raisebox{50pt}{\rotatebox[origin=c]{90}{\textsc{Tail}}}} \hspace{-7pt} &
        % \animage{0 0 0 0}{toby-tail1.train.jpg} &
        % \animage{0 0 0 0}{toby-tail1.valid.jpg} &
        % \textimage{0 0 0 0}{toby-tail1.full_model_se3_w0.01.pred.jpg}{25.1}{\bestnum{0.127}} &
        % \textimage{0 0 0 0}{toby-tail1.d-nerf.pred.jpg}{\bestnum{26.9}}{0.353} &
        % \textimage{0 0 0 0}{toby-tail1.nsff.pred.jpg}{24.0}{0.385} &
        % \textimage{0 0 0 0}{toby-tail1.neuralvolumes.pred.jpg}{16.5}{0.462} &
        % \textimage{0 0 0 0}{toby-tail1.nerf.pred.jpg}{22.8}{0.506} \\
               
        % \makebox[20pt]{\raisebox{45pt}{\rotatebox[origin=c]{90}{\textsc{Broom}}}} \hspace{-7pt} &
        % \animage{60 80 00 50}{broom2.train.jpg} &
        % \animage{30 80 30 50}{broom2.valid.jpg} &
        % \textimage{30 80 30 50}{broom2.full_model_se3_w0.01.pred.jpg}{20.7}{\bestnum{0.240}} &
        % \textimage{30 80 30 50}{broom2.d-nerf.pred.jpg}{\bestnum{22.8}}{0.600} &
        % \textimage{30 80 30 50}{broom2.nsff.pred.jpg}{21.8}{0.306} &
        % \textimage{30 80 30 50}{broom2.neuralvolumes.pred.jpg}{{14.2}}{0.472} &
        % \textimage{30 80 30 50}{broom2.nerf.pred.jpg}{18.7}{0.677} \\
 
    
        \\[2pt]
        
        & {\small Training view} & 
        {\small Novel view (GT)} & 
        {\small Ours} &
        {\small $\gamma$(t)+trans} &
        {\small NSFF~\cite{li2020neural}} &
        {\small NV~\cite{lombardi2019neural}} &
        {\small NeRF~\cite{mildenhall2020nerf}}
        \\
    \end{tabular}
    \vspace{-6pt}
    \caption{Comparisons of baselines and our method. {\footnotesize PSNR / LPIPS} metrics on bottom right with best colored \bestnum{red}.}
    \label{fig:additional-vrig-results}
    \vspace{-12pt}
\end{figure*}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
